Iris Recognition for Infants

Non-invasive, efficient, physical token-less, accurate and stable identification methods for newborns may prevent baby swapping at birth, limit baby abductions and improve post-natal health monitoring across geographies, within the context of both the formal (i.e., hospitals) and informal (i.e., humanitarian and fragile settings) health sectors. This paper explores the feasibility of application iris recognition to build biometric identifiers for 4-6 week old infants. We (a) collected near infrared (NIR) iris images from 17 infants using a specially-designed NIR iris sensor; (b) evaluated six iris recognition methods to assess readiness of the state-of-the-art iris recognition to be applied to newborns and infants; (c) proposed a new segmentation model that correctly detects iris texture within infants iris images, and coupled it with several iris texture encoding approaches to offer, to the first of our knowledge, a fully-operational infant iris recognition system; and, (d) trained a StyleGAN-based model to synthesize iris images mimicking samples acquired from infants to deliver to the research community privacy-safe infant iris images. The proposed system, incorporating the specially-designed iris sensor and segmenter, and applied to the collected infant iris samples, achieved Equal Error Rate (EER) of 3\% and Area Under ROC Curve (AUC) of 99\%, compared to EER$\geq$20\% and AUC$\leq$88\% obtained for state of the art adult iris recognition systems. This suggests that it may be feasible to design methods that succesfully extract biometric features from infant irises.

==> figure-tex/genuin-synthetic-score-distribution.tex <==
\begin{figure}[htb!] 
    \centering
    \begin{subfigure}[b]{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/HDBIF-Syn-Gen-dist.pdf}
        \caption{HDBIF Normalized}
        \label{score-dist:hdbif-gen-syn}
    \end{subfigure}%
    \begin{subfigure}[b]{0.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/DGR-Syn-Gen-dist.pdf}
        \caption{DGR Normalized}
        \label{score-dist:dgr-gen-syn}
    \end{subfigure}%

    \caption{Distribution of genuine and impostor scores for the HDBIF and DGR iris recognition matchers. The impostor scores are obtained from matching genuine irises with synthetic irises.}
    \label{fig:gen-syn-score-distribution} 
\end{figure}

==> figure-tex/roc-curve.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/roc_curve.pdf}

    \caption{ROC curve for different iris recognition matchers, plotting True Match Rate (TMR) against False Match Rate (FMR). Each matcher is indicated with its Equal Error Rate (EER) and Area Under the Curve (AUC) values. Vanilla models use the original segmentation approach, while Norm models use our proposed segmentation approach. The high AUC and low EER values demonstrate the superior performance of the Norm models over the vanilla models.}

    \label{fig:roc-curve}
\end{figure}
